Deterministic Performance Analysis of Subspace Methods for Cisoid Parameter Estimation

Performance analyses of subspace algorithms for cisoid parameter estimation available in the literature are predominantly of statistical nature with a focus on asymptotic$-$either in the sample size or the SNR$-$statements. This paper presents a deterministic, finite sample size, and finite-SNR performance analysis of the ESPRIT algorithm and the matrix pencil method. Our results are based, inter alia, on a new upper bound on the condition number of Vandermonde matrices with nodes inside the unit disk. This bound is obtained through a generalization of Hilbert's inequality frequently used in large sieve theory.

==> def.tex <==
% !TEX root = isit16_submeth.tex

% To define macros
\makeatletter
\def\iffirsttoken#1#2{
	\expandafter\def\expandafter\@first@token\expandafter{\@car#1\@nil}
	\expandafter\ifx\@first@token#2\relax
	\expandafter\@firstoftwo
 \else
  	\expandafter\@secondoftwo
 \fi
}


% Theorems
\newtheorem{thm}{Theorem}
\newtheorem{cor}[thm]{Corollary}   % Turned off theorem numbering
\newtheorem{prop}{Proposition}
\newtheorem{defn}{Definition}
\newtheorem{ex}{Example}
\newtheorem{lem}[thm]{Lemma}

% Triangleq
\renewcommand{\triangleq}{\vcentcolon=}
\newcommand{\reversetriangleq}{=\vcentcolon}

% Sets
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\torus}{\mathbb{T}}

% Inequalities
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}

% Functions
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\abs}[1]{\left| #1 \right|}
\DeclareMathOperator{\sh}{sh}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\colsp}{colsp}
\DeclareMathOperator{\rowsp}{rowsp}
\DeclareMathOperator{\tr}{tr}

% Real and imaginary parts
\newcommand{\real}{\mathfrak{Re}}
\newcommand{\imag}{\mathfrak{Im}}
\renewcommand{\Re}[1]{\real\left\{#1\right\}}
\renewcommand{\Im}[1]{\imag\left\{#1\right\}}

% Notation
\newcommand{\vandermonde}[2]{\boldsymbol{\mathscr{V}}_{\!#1}(#2)}
\newcommand{\hankel}[2]{\boldsymbol{\mathscr{H}}_{\!#1}(#2)}
\newcommand{\sig}{x}
\newcommand{\sigVector}{\boldsymbol{x}}
\newcommand{\noisySig}{\widetilde{\sig}}
\newcommand{\noisySigVector}{\widetilde{\sigVector}}
\newcommand{\node}{z}
\newcommand{\nodeVector}{\boldsymbol{z}}
\newcommand{\nbNodes}{K}
\newcommand{\nbSamples}{N}
\newcommand{\weight}{\alpha}
\newcommand{\weightVector}{\boldsymbol{\weight}}
\newcommand{\noise}{e}
\newcommand{\noiseVector}{\boldsymbol{\noise}}
\newcommand{\sizeData}{L}
\newcommand{\dataMatrix}{\mathbf{X}}
\newcommand{\noisyDataMatrix}{\widetilde{\dataMatrix}}
\newcommand{\corrMatrix}{\mathbf{C}_\dataMatrix}
\newcommand{\noiseMatrix}{\mathbf{E}}
\newcommand{\noisyDataMatrixOne}{\widetilde{\mathbf{X}}_{1}}
\newcommand{\noisyDataMatrixTwo}{\widetilde{\mathbf{X}}_{2}}
\newcommand{\noiseMatrixOne}{\mathbf{E}_1}
\newcommand{\noiseMatrixTwo}{\mathbf{E}_2}
\newcommand{\dataMatrixOne}{\mathbf{X}_1}
\newcommand{\dataMatrixTwo}{\mathbf{X}_2}


\newcommand{\vander}{\mathbf{V}}
\newcommand{\diagNodes}{\mathbf{D}_z}
\newcommand{\diagCoeff}{\mathbf{D}_\alpha}

\newcommand{\matA}{\mathbf{A}}
\newcommand{\matB}{\mathbf{B}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\matId}{\mathbf{I}}
\newcommand{\matU}{\mathbf{U}}

\newcommand{\subspaceMatrix}{\mathbf{S}}
\newcommand{\noiseSubspaceMatrix}{\subspaceMatrix_\perp}
\newcommand{\subspace}{\mathcal{S}}
\newcommand{\noisySubspaceMatrix}{\widetilde{\mathbf{S}}}
\newcommand{\noisyNoiseSubspaceMatrix}{\noisySubspaceMatrix_\perp}



==> previousWork.tex <==
% !TEX root = isit16_submeth.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Relation to previous work
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Relation to previous work}

%\cite{Kot1993} 
%\cite{Porat1987} 
%\cite{Okkovat1989}


In \cite{Eriksson1993} and \cite{Stoica1991}, it is shown that in the case of undamped sinusoids, LS-ESPRIT has an asymptotic efficiency close to $1$ under the assumptions $\mathrm{SNR} \rightarrow \infty$ and $N \rightarrow \infty$, respectively.  
In \cite{Rao1988}, expressions for the asymptotic mean squared error in the estimates of the direction of arrival are derived for LS-ESPRIT and TLS-ESPRIT. Moreover, it is shown that, asymptotically, the estimates obtained using these both variants of the ESPRIT algorithm have the same mean squared error. In \cite{Ottersten1991}, the asymptotic distribution of the estimation error for TLS-ESPRIT is derived. Both \cite{Rao1988} and \cite{Ottersten1991} assume a linear equispaced array and jointly complex Gaussian sources in additive white Gaussian noise. In \cite{Yuen1996}, the analysis of \cite{Rao1988} is generalized to non-Gaussian sources.
In \cite{Hua1991}, it is shown that in the case of undamped sinudoids, the matrix pencil method and the ESPRIT algorithms are less sensitive to noise than MUSIC. \cite{Li1991} proposes a unified performance analysis which is applicable to both LS-ESPRIT and the matrix pencil algorithm under the assumption $\mathrm{SNR} \rightarrow \infty$.

In \cite{Hua1988, Hua1990}, Hua and Sarkar present a first-order perturbation analysis of the matrix pencil method and compares the performance of matrix pencil method to the one of a variant of the Prony method. This analysis is valid at high SNR, only.
In \cite{Rio1996}, the performance of the matrix pencil method is compared to the Fourier transform technique for the estimation of undamped sinusoids.
The paper \cite{Djermoune2004} gives an estimation performance in the case of a single exponentially damped sinusoid and compare it to the performance of the Kumaresan-Tufts method.

Moitra~\cite{Moitra2014} provides a performance analysis for a modified matrix pencil method, that is, modified in the sense that he builds the matrices $\mathbf{A} = \vander_L\mathbf{D}_\alpha\vander_L^H$ and $\mathbf{B} = \vander_L\mathbf{D}_{\boldsymbol{\alpha}}\mathbf{D}_{\boldsymbol{z}}\vander_L^H$ instead of building the Hankel matrices $\dataMatrixOne$ and $\dataMatrixTwo$. He then looks for the generalized eigenvalues of $(\mathbf{A}, \mathbf{B})$, which are $\node_1, \node_2, \ldots, \node_\nbNodes$ in the case where $\abs{\node_k} = 1$ for all $k \fromto{1, 2, \ldots, \nbNodes}$. If the nodes $\node_1, \node_2, \ldots, \node_\nbNodes$ are in the unit disk, not necessarily on the unit circle, we could also use such a method and look for the generalized eigenvalues of $(\mathbf{A}, \mathbf{B})$, with $\mathbf{A} = \vander_L{\node_1, \node_2, \ldots, \node_\nbNodes}\mathbf{D}_{\boldsymbol{\alpha}}\vander_L'$ and $\mathbf{B} = \vander_L\mathbf{D}_{\boldsymbol{\alpha}}\mathbf{D}_{\boldsymbol{z}}\vander_L'$, with $\vander_L'$ been the $L \times \nbNodes$ Vandermonde matrix with nodes $\node_1^{-1}, \node_2^{-1}, \ldots, \node_\nbNodes^{-1}$, instead of those of $(\dataMatrixOne, \dataMatrixTwo)$. However, the performance analysis given in \cite{Moitra2014} does only hold for undamped sinusoids, i.e., in  the case where $\abs{\node_k} = 1$ for all $k \fromto{1, 2, \ldots, \nbNodes}$, as it depends on the condition number of $\vander_L$ for which Moitra establishes an upper bound that holds in this case only.

